Parallel training of linear models without compromising convergence

In this paper we analyze, evaluate, and improve the performance of training generalized linear models on modern CPUs. We start with a state-of-the-art asynchronous parallel training algorithm, identify system-level performance bottlenecks, and apply optimizations that improve data parallelism, cache line locality, and cache line prefetching of the algorithm. These modifications reduce the per-epoch run-time significantly, but take a toll on algorithm convergence in terms of the required number of epochs. To alleviate these shortcomings of our systems-optimized version, we propose a novel, dynamic data partitioning scheme across threads which allows us to approach the convergence of the sequential version. The combined set of optimizations result in a consistent bottom line speedup in convergence of up to 12x compared to the initial asynchronous parallel training algorithm and up to 42x, compared to state of the art implementations (scikit-learn and h2o) on a range of multi-core CPU architectures.

==> background.tex <==
% !TEX root = paper.tex

\section{Background}

Our optimizations involve marrying ideas from parallel and distributed learning to optimally leveraging system resources at multiple levels.


\paragraph{Parallel Coordinate Descent}

% introduce problem with shared vector

Parallel algorithms are based on the availability of shared memory between cores.
Previous approaches for scaling up stochastic coordinate descent methods to more than one core \cite{liu2015asynchronous, Hsieh2015, Tran2015} follow roughly the same pattern: the algorithm is implemented \textit{asynchronously} using multiple threads, whereby each thread is assigned a different coordinate to update. Such an approach enables the parallel execution of multiple updates to better utilize compute resources. 

It has been shown in \cite{Hsieh2015, Tran2015,sdca2013} that keeping auxiliary information in memory to avoid recurring computations can significantly reduce the update complexity of the algorithm. However for asynchronous implementations this can lead to write contention problems.

Depending on how this is solved it can lead to divergence of asynchronous algorithm. 
Thus the scalability of asynchronous algorithms is limited.


\CDU{should I add the pseudo-code of the algorithm we start from?}

\paragraph{Distributed Learning}
 Distributed algorithms are designed for a data parallel setting, where the training data is partitioned across the worker nodes in a cluster. The assumption is that moving data over the network is very expensive. To this end, algorithms like CoCoA~\cite{cocoa18jmlr} attempt to pair good convergence guarantees with efficient distributed communication. They define data-local problems that can be operated on in parallel by the different workers and define a shared vector that is periodically exchanged over the network to synchronize their work. The algorithm is theoretically sound and can be scaled to an arbitrary number of nodes.
However convergence suffers when more nodes are added.



==> related.tex <==
\section{Related Work}


